Probing Contextual Diversity for Dense Out-of-Distribution Detection

Detection of out-of-distribution (OoD) samples in the context of image classification has recently become an area of interest and active study, along with the topic of uncertainty estimation, to which it is closely related. In this paper we explore the task of OoD segmentation, which has been studied less than its classification counterpart and presents additional challenges. Segmentation is a dense prediction task for which the model's outcome for each pixel depends on its surroundings. The receptive field and the reliance on context play a role for distinguishing different classes and, correspondingly, for spotting OoD entities. We introduce MOoSe, an efficient strategy to leverage the various levels of context represented within semantic segmentation models and show that even a simple aggregation of multi-scale representations has consistently positive effects on OoD detection and uncertainty estimation.

==> tables/single_dilation.tex <==
\begin{table}
\centering
\small
\begin{tabular}{l|rrrr|r}
\toprule
                & \rotatebox{0}{SD} & \rotatebox{0}{SD} & \rotatebox{0}{SD} & \rotatebox{0}{SD} & \rotatebox{0}{MD} \\
                & \rotatebox{0}{1} & \rotatebox{0}{12} & \rotatebox{0}{24} & \rotatebox{0}{36} & \rotatebox{0}{MOoSe} \\ 
                \midrule
\globalhead     & 8.20                     & 8.05                     & 9.13                     & 8.58                      & 10.23                     \\
+ probes & 10.06                   & 10.06                    & 10.63                    & 10.49                     & 13.08                     \\
\midrule
Change          & 1.86                    & 2.01                     & 1.50                      & 1.91                      & 2.85                      \\
Change \%       & 22.68                   & 24.97                    & 16.43                    & 22.26                     & 27.86         \\
\bottomrule
\end{tabular}
\caption{\textbf{Single-Dilation ablation.} OoD detection results (AUPR) for single dilation models (SD) with different dilation rates (1, 12, 24, 36), compared to standard (multi-dilation, MD) \modelname. First row shows results for the global head, second row adds the probes, bottom two rows show the absolute and relative improvement.}
\label{tab:single_dilation}
\end{table}
